Randomised Rounding with Applications

We develop new techniques for rounding packing integer programs using iterative randomized rounding. It is based on a novel application of multidimensional Brownian motion in $\mathbb{R}^n$. Let $\overset{\sim}{x} \in {[0,1]}^n$ be a fractional feasible solution of a packing constraint $A x \leq 1,\ \ $ $A \in {\{0,1 \}}^{m\times n}$ that maximizes a linear objective function. The independent randomized rounding method of Raghavan-Thompson rounds each variable $x_i$ to 1 with probability $\overset{\sim}{x_i}$ and 0 otherwise. The expected value of the rounded objective function matches the fractional optimum and no constraint is violated by more than $O(\frac{\log m} {\log\log m})$.In contrast, our algorithm iteratively transforms $\overset{\sim}{x}$ to $\hat{x} \in {\{ 0,1\}}^{n}$ using a random walk, such that the expected values of $\hat{x}_i$'s are consistent with the Raghavan-Thompson rounding. In addition, it gives us intermediate values $x'$ which can then be used to bias the rounding towards a superior solution.The reduced dependencies between the constraints of the sparser system can be exploited using {\it Lovasz Local Lemma}. For $m$ randomly chosen packing constraints in $n$ variables, with $k$ variables in each inequality, the constraints are satisfied within $O(\frac{\log (mkp\log m/n) }{\log\log (mkp\log m/n)})$ with high probability where $p$ is the ratio between the maximum and minimum coefficients of the linear objective function. Further, we explore trade-offs between approximation factors and error, and present applications to well-known problems like circuit-switching, maximum independent set of rectangles and hypergraph $b$-matching. Our methods apply to the weighted instances of the problems and are likely to lead to better insights for even dependent rounding.

==> concl.tex <==
\section{Concluding Remarks}




==> genapprox.tex <==
\subsection{A general approximation bound :Proof of theorem \ref{mainthm3}}

If we are interested in maintaining feasibility of constraints, we can
ensure it by sacrificing the value of the objective function according to
some trade-offs. The same algorithm works, where we use the known method 
of damping the probabilities of rounding (\cite{RT:87,AS:95}).

Let $X_1 , X_2 \ldots X_u$ denote the unabsorbed random 
variables in a constraint
after the Brownian walk phase and let $ U = \sum_i X_i  = \frac{B}{\beta}$
for some $\beta \geq 1$. Let $\hat{X_i}$ be the $\{0, 1\}$ random variables
where $\Pr [ \hat{X_i} =1] = X_i$ and so $\E [ \sum_i  \hat{X_i} ] = 
\sum_i X_i = \frac{B}{\beta}$. To apply LLL, we need
$\Pr [ \sum_i \hat{X_i} > B ] < \frac{1}{d}$.

Since $U = \sum_i \hat{X_i}$, then from Chernoff bounds, we know that 
\begin{equation}
 \Pr [ U \geq (1+ \Delta)\E[ U ] \leq {\left[ \frac{e^\Delta }{ { (1+ 
\Delta )}^{ 1+ \Delta }} \right]}^{E[U]} 
\label{chernoff}
\end{equation}
Using $\E [ U ] = \frac{B}{\beta}$ and $\beta = 1+ \Delta $ we obtain
$\Pr [ U \geq B ] \leq {\left[ \frac{e^{\beta -1}}{ {(\beta )}^{\beta}}\right]
}^{B/\beta} \leq {\left( \frac{e}{\beta} \right)}^B \leq \frac{1}{\alpha d}$
for some scale parameter $\alpha \geq 1$.
It follows that 
\begin{equation}
 {( \beta /e )}^{B} > d\alpha 
\label{damp_req}
\end{equation}
Therefore $\beta = e {(d \alpha)}^{1/B}$.
Since our matrices are 0-1, the
minimum infeasibility happens at $B+1$, so we can substitute $B+1$ instead
of $B$ in the previous calculations to obtain $\beta = e {(d \alpha)}^{1/B+1}$.  
Using $S \geq 1$ as the initial scaling for Brownian walk,
we obtain the following result using Lemma \ref{err_bnd}
\begin{lemma}
For $S \geq c'\cdot {(d\alpha )}^{1/(B+1)}$ , and $B \geq 1$,
we can round the fractional solution to a feasible integral solution
with objective function value $\Omega ( OPT /S )$ for $OPT \geq \Omega 
( mS/(\alpha d)))$. 
\label{colbndapprox}
\end{lemma}
 The last condition in the Lemma follows since Equation (\ref{eqnobj}) is 
satisfied. 

It would be worthwhile to compare and contrast our results and techniques
with \cite{AS:95,AS:96}. For the case of the number of 1's bounded
by $\rho$ in a 0-1 matrix\footnote{Our techniques and proofs must be
modified to work for more general matrices having entries from $[0,1]$} $A$, an objective value $OPT/ {\rho}^{1/B}$  
was obtained which is marginally superior to our result of
$OPT/{(\rho \log n)}^{1/(B+1)}$.
Still, we believe, that our techniques are 
easier to use and build upon for various applications compared to the FKG
inequality based techniques. Following the Brownian motion, the number
of non-zero coefficients in any constraint is at most $O(\log n)$ but it
is not clear how this can be exploited by FKG based analysis of \cite{AS:95,
BS:00} which is independent of the number of columns.

For weighted objective function with $c_i \geq 1/p$, we can choose
the value of the scaling factor $\alpha$ more carefully so that $p =
\alpha^{1 - 1/B'} \cdot {(\log n)}^{1 -2/B'} $, and $mk/n \leq \log m$,
using $S = {(\alpha \log^2 n )}^{1/B'}$ gives an objective value
of at least $ nB'/(p Sk)  \geq n/(k \alpha \log n) $
which satisfies condition \ref{eqnobj}. Note that $S = {( p \log n)}^{1/(B'-1)}
$ from the above parameter settings.\\
%For $B = 1$, the scaling function is undefined. However, for the
%case $A_{i,j} \in \{ 0, 1\}$, we observe that a constraint is infeasible for
%error $\geq B+1$ since it cannot take any values between $B$ and $B+1$.
By subsituting back $B+1$ for $B'$ in the previous calculations,
$S = {( p \log n)}^{1/B}$. So for $B = 1$, the approximation is
$O(p\log n)$.
%values consistent with condition \ref{eqnobj}.
%we set $\alpha = \log n$ giving $S = \log^3 n$. Then the
%objective function value is $n/(k \log^3 n)$ which satisfies
This completes the proof of Theorem \ref{mainthm2}. \\[0.1in]


==> lbnd.tex <==
\subsection{A Lower Bound on error}
\begin{lemma}
For $A \in {\cal A}^{m\times n}_{\log n}$ such that $A\cdot \bar{x} \leq e^m$,
we cannot simultaneously obtain $\sum_i \hat{x}_i = \Omega ( n/\log n )$ and
${|| A \hat{x}||}_\infty  \leq o(\frac{\log\log n}{\log\log\log n})$
for $\hat{x}_i \in \{ 0, 1 \}$.
\label{lbnd}
\end{lemma}

\begin{proof}

As mentioned before, it is easy to see that $x_i = 1/k$ is a solution 
for $\bar{x}$ with objective
function value $n/k$. After rounding $\bar{x}$ we want to have at least 
$\Omega ( n/k )$ 1s in the rounded vector, say $\bar{y}$.
%\todo{Actually the expectation is $n/k$ or $n/k$ with some probability 1/2} 
We must have $A \cdot \bar{y} \leq t\cdot e$ for some rounding guarantee
$t$. Let $b$ be a fixed vector with $n/k$ 1s. 

Let $r$ be a row vector with $k$ 1s in random location - this corresponds to
a row of $A$. The probability that $< r , \bar{y} > \ \ \geq t$ is given by
 \[  \frac{{ (n/k) \choose t} 
\cdot { (n-n/k) \choose (k-t) }}{{n \choose k }} \]
Using $ {(\frac{n}{k})}^k \leq {n \choose k} \leq {(\frac{ne}{k})}^k $, the 
above expression is
\begin{eqnarray}
 \geq & \frac{ {( \frac{n}{tk})}^t \cdot {(\frac{n -n/k}{k-t})}^{k-t}}{
{(\frac{ne}{k})}^k} \\
 = & \frac{ \frac{1}{t^t} \cdot {( \frac{k-1}{k-t})}^{k-t}} {
 e^k } \\ 
 = & \frac{ k^{k-t}}{ {( k-t )}^{k-t} \cdot e^k \cdot t^t }\\
 = & \frac{1}{ {( 1 - t/k )}^{k-t} \cdot e^k \cdot t^t } \\
 \geq & \frac{1}{{( 1 - t/k )}^{k/2} \cdot e^k \cdot t^t } \text{ for } k \gg t\\
 = & \frac{1}{ e^{ k - t/2} \cdot t^t }
\end{eqnarray}
So the probability that for $m$ independently chosen rows, the probability that
$< r , \bar{y} > \ \ < t$ is 
\begin{eqnarray}
  p(m,k,t) &  \leq & {\left( 1 - \frac{1}{ e^{ k - t/2} \cdot t^t } \right)}^m 
\leq  {\left( 1 - \frac{1}{ e^{ k } \cdot t^t } \right)}^m =
{\left( 1 - \frac{1}{ e^{ k } \cdot t^t } \right)}^{e^k t^t \frac{m}{e^k t^t}}
\\
 & \leq & {\left( \frac{1}{e} \right)}^{\frac{m}{e^k t^t}} 
\end{eqnarray} 
Since there are no more than ${n \choose
(n/\log n)}$ choice of columns with $n/\log n$ 1s, the probability that all
the dot products are less than $t$ is less than ${n \choose (n/\log n)} \cdot
p(m,k,t)  \leq p(m,k,t) \cdot {(\frac {n e}{n/\log n})}^{n/\log n} 
 \leq e^n \cdot p(m,k,t)$. If $e^n \cdot p(m,k,t) < 1$ then there must exist
matrices in ${\cal A}^{m \times n}_k$ that do not satisfy the error bound $t$.
So,
\[    1  > {\left( \frac{1}{e} \right)}^{\frac{m}{e^k t^t}} \cdot e^{n} 
    \Rightarrow {( e ) }^{\frac{m}{e^k t^t}}  >  e^n \] 
 which is equivalent to the condition 
\begin{equation}
 \frac{m}{n}  > e^k t^t \text{  or  }
\log(m/n) > k + t\log t 
\label{lbndreq}
\end{equation}
 
 For $k = \log n$ and $m = n\cdot polylog(n) $, this holds for some $t \geq 
\frac{\alpha \log \log n}{\log\log\log n})$, i.e., for some constant 
$\alpha > 0$, i.e., 
the error cannot be
$o (\frac{\log\log n}{\log\log\log n})$. 
\end{proof}
%Note that for $t \geq 
%c \frac{\log n}{\log\log n}$ this can be avoided for any polynomial
%sized $m$ by choosing an appropriately large $c$. 

%{\it Remark} In general if we compare the bound in Theorem \ref{randmaterr}
%and Equation \ref{lbndreq}, the bound on $t$ is nearly tight, namely
%for error $t = \Theta ( \frac{\log(m/n)}{log\log (m/n)})$, it is achievable
%by our algorithm, as well as, it cannot be refuted using $m = n^{O(1)}$.
%\todo{The term $e^k$ comes from Stirlings approximation and seems to explain
%the difference between lower and upper bound}.
%{\bf $p(m,c )$ ?} It is simplistic to compute $p(m,c)$ by multiplying the
%independent probabilities since that doesn't take care of duplicate rows.
%Out of the total of ${n_k}$ rows with $k$ 1s ($n_k = {n \choose k}$), 
%we need to estimate 
%the number of {\em good } rows, say $n_g$. We will pick
%$m$ rows from $n_g$ rows. The probability that a matrix is {\em good} for 
%a fixed vector $b$ =
%\[ \frac{ {n_g \choose m}}{{ n_k \choose m}}  \leq \frac{ { n_g }^m}{
 %{ ( n_k /e)}^m}\]
%Unless $ n_g \leq n_k /e$, this ratio is not less than 1. This is much less
%than $(1 - 1/ polylog (n) )$, the best that we can hope to prove for the
%range of values we are interested in.
%}


==> lllgen.tex <==
\subsection{A general approximation bound }

If we are interested in maintaining feasibility of constraints, we can
ensure it by sacrificing the value of the objective function according to
some trade-offs. The same algorithm works, where we use the known method 
of damping the probabilities of rounding (\cite{RT:87,AS:95}).

Let $X_1 , X_2 \ldots X_u$ denote the unabsorbed random 
variables in a constraint
after the Brownan motion phase and let $ U = \sum_i X_i  = \frac{B}{\beta}$
for some $\beta \geq 1$. Let $\hat{X_i}$ be the $\{0, 1\}$ random variables
where $\Pr [ \hat{X_i} =1] = X_i$ and so $\E [ \sum_i [ \hat{X_i} ] = 
\sum_i X_i = \frac{B}{\beta}$. To apply LLL, we need
$\Pr [ \sum_i \hat{X_i} > B ] < \frac{1}{d}$.

Since $U = \sum_i \hat{X_i}$, then from Chernoff bounds, we know that 
\begin{equation}
 \Pr [ U \geq (1+ \Delta)\E[ U ] \leq {\left[ \frac{e^\Delta }{ { (1+ 
\Delta )}^{ 1+ \Delta }} \right]}^{E[U]} 
\label{chernoff}
\end{equation}
Using $\E [ U ] = \frac{B}{\beta}$ and $\beta = 1+ \Delta $ we obtain
$\Pr [ U \geq B ] \leq {\left[ \frac{e^{\beta -1}}{ {(\beta )}^{\beta}}\right]
}^{B/\beta} \leq {\left( \frac{e}{\beta} \right)}^B \leq \frac{1}{\alpha d}$
for some scale parameter $\alpha \geq 1$.
It follows that 
\begin{equation}
 {( \beta /e )}^{B} > d\alpha 
\label{damp_req}
\end{equation}
Therefore $\beta = e {(d \alpha)}^{1/B}$.
Using $S \geq 1$ as the initial scaling for Brownian motion,
we can obtain the following result using Lemma \ref{err_bnd}
\begin{lemma}
For $S \geq c'\cdot {(d\alpha )}^{1/B}$ , and $B \geq 1$,
we can round the fractional solution to a feasible integral solution
with objective function value $\Omega ( OPT /S )$ for $OPT \geq \Omega 
( mS/(\alpha d)))$. 
\label{colbndapprox}
\end{lemma}
 The last condition in the Lemma follows from Equation \ref{eqnobj} is 
satisfied. 
This completes the proof of Theorem \ref{mainthm2}.

It would be worthwhile to compare and contrast our results and technqiues
with \cite{AS:95,AS:96}. For the case of the number of 1's bounded
by $\rho$ in a 0-1 matrix $A$, an objective value $OPT/ {\rho}^{1/B}$  
is obtained which is marginally superior to our result of
$OPT/{(\rho \log n)}^{1/B}$. Still, we believe, that our technqiues are 
easier to use and build upon for various applications compared to the FKG
inequality based technqiues. Following the Brownian motion, the number
of non-zero coefficients in any constraint is at most $O(\log n)$ but it
is not clear how this can be capitalized by FKG based analysis.

%\noindent{\bf Remark} If we apply the LLL directly, then $d = \rho k$ and the 
%scaling is actually $S = {( \rho k )}^{1/B}$ which could be significantly
%larger (and the objective function is smaller) for $k \gg \log n$.

